Correctness is not Faithfulness in RAG Attributions

Retrieving relevant context is a common approach to reduce hallucinations and enhance answer reliability. Explicitly citing source documents allows users to verify generated responses and increases trust. Prior work largely evaluates citation correctness - whether cited documents support the corresponding statements. But citation correctness alone is insufficient. To establish trust in attributed answers, we must examine both citation correctness and citation faithfulness. In this work, we first disentangle the notions of citation correctness and faithfulness, which have been applied inconsistently in previous studies. Faithfulness ensures that the model's reliance on cited documents is genuine, reflecting actual reference use rather than superficial alignment with prior beliefs, which we call post-rationalization. We design an experiment that reveals the prevalent issue of post-rationalization, which undermines reliable attribution and may result in misplaced trust. Our findings suggest that current attributed answers often lack citation faithfulness (up to 57 percent of the citations), highlighting the need to evaluate correctness and faithfulness for trustworthy attribution in language models.

==> figures/colorboxes/citation_example.tex <==
\begin{tcolorbox}[title=Example Citation]
\textbf{Question}: how long was gabby in a coma in the choice \\
\textbf{Grounded answer}: In the <co: 0,4>novel</co: 0,4> *<co: 0,3,4>The Choice</co: 0,3,4>*, Gabby is in a coma for <co: 0>three months.</co: 0> 
\\ 

Document 0: Contains the three-month coma and the word novel as well as the title "The Choice" \\
Document 1: Contains the title "The Choice" but is not cited\\ 
Document 2: Contains the title "The Choice" but is not cited\\
Document 3: Contains the title "The Choice" and \textbf{is} cited\\ 
Document 4: Contains the title "The Choice" and the word novel and \textbf{is} cited
\end{tcolorbox}
